Taking Informed Action on Student Activity in MOOCs

This paper presents a novel approach to understand specific student behavior in MOOCs. Instructors currently perceive participants only as one homogeneous group. In order to improve learning outcomes, they encourage students to get active in the discussion forum and remind them of approaching deadlines. While these actions are most likely helpful, their actual impact is often not measured. Additionally, it is uncertain whether such generic approaches sometimes cause the opposite effect, as some participants are bothered with irrelevant information. On the basis of fine granular events emitted by our learning platform, we derive metrics and enable teachers to employ clustering, in order to divide the vast field of participants into meaningful subgroups to be addressed individually.

==> sections/implementation.tex <==
%!TEX root = ../cluster.tex

\section{Implementation}
Prior to implementing ``Cluster Viewer'', two requirements were defined:
exploration of possible groups in a course should be enabled directly on the platform;
instructors shall be given the possibility to interactively analyze activity along the metrics based on their intuition and experience.
%TODO: Footnote: Xikolo?
Given those prerequisites, we decided to integrate parts of the software directly within the micro-services of our MOOC platform (xikolo), and to attach an R-server for the clustering and evaluation tasks.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{gfx/architecture-overview}
  \caption{The openHPI architecture with a focus on the analytics service for the task of cluster analysis.}
  \label{fig:architecture-overview}
\end{figure}

%% TODO: reference master thesis!!

Figure \ref{fig:architecture-overview} shows the most important services that contribute to fulfill the posed requirements.

The \emph{web} service builds the user frontend and aggregates data from other services to allow for a coherent and rich presentation of the potential clusters.
The actual calculation is done inside the analytics service.
Whenever a clustering request is issued by the user via the frontend (i.e. the web service), the \emph{QueryController} class takes part in handling this request.
It interacts with the \emph{Dimensions} class to aggregate the desired metrics, which itself retrieves the required data from the underlying postgres database.
The Dimensions class holds specific queries for the pre-defined metrics that combine several of the base events.
Whenever a new metric should be added, this class can be easily adapted.
Aggregated data from the Dimensions class is passed to the Clusterer class that feeds it into the R-Server, carrying out the actual calculations.
While our current setup stores all necessary event data in a postgres database, the analytics service also supports to query neo4J or ElasticSearch data sources.

\subsection{Metric computation}
%TODO: Obligatory?
The event data used for the clustering has a defined obligatory minimal structure and additional optional elements.
Each element comes with the user ID of the participant issuing the event, the verb (or name of the event), and a resource ID.
Optional elements might include additional context and result information.
%MAYBE TOO MUCH DETAIL
%Events are either collected directly or indirectly.
%The events are directly send from the web-frontend (i.e. the web-service) to the analytics service if their information does not need to be validated by another service. An example for this is the download of some slides, which is self-sufficient in the web-service.
%Other activities, like the creation of a new thread in the forum, is cross-validated with the pinboard service, and then issued from the pinboard service to the analytics service.

%\subsection{Metric computation}

As mentioned in the Section \ref{sec:concept}, metrics combine several events to a more general or better graspable value.
Discovery metrics, for example, subsume visits of distinct resources, while performance metrics average the results of submitted assignments.
% TODO: Should we talk about tables?
The metrics thus rely on manually written SQL queries that simply join the participating tables in order to create the outcome as a single combined numerical value per metric and user.
To speed up response times and to better utilize our system resources, we combine all requested metrics to one concatenated query using SQL joins.
Thus we need only one round trip to the data source.
The extracted metrics are all numeric and returned as a vector per user  $u = \{v_{1}, \dots ,v_{m} \}$ with $m$ values, one per computed metric.
The result set of $n$ valid users thus forms a matrix $D_{n,m} $, containing the value of each metric for each valid user and being the starting point for the cluster analysis.
% TODO: Delete sentence below?
In order to simplify the results, we only expose those rows, where at least one metric has a value differing from zero.

\subsection{Clustering}
  \label{sec:clustering}
%After choosing the R server to be the component to be the clustering
%TODO: QUellen auf Seite 29 der MA nutzen in Related work???

%TODO: Check rserve-client url (maybe without version?)
The analytics service, written in Ruby on Rails, communicates with the R server using \emph{Rserve}\footnote{\url{https://rforge.net/Rserve/}} and the Ruby gem \emph{rserve-client}\footnote{\url{https://rubygems.org/gems/rserve-client/versions/0.3.1}}.
Once the data has been transferred by the \emph{QueryController}, we employ K-Means \cite{hartigan1979algorithm} to create clusters representing potentially meaningful student groups.
Other distance-baseed clustering approaches like hierarchical clustering or density based clustering were evaluated but rejected due to their increased runtime (>10 seconds) for participant volumes of over 15,000 users per course preventing for interactive exploration.

The steps to build the clusters consist of the following:

\begin{itemize}
\item data normalization: data from different input dimensions needs to be normalized to a common domain in order not to distort the results of the distance-based K-Means clustering.
For that, we use R's scale method.
\item cluster estimation: K-Means needs the desired number of clusters as input.
Thus, we use partitioning around medoids (R's pamk-method) to perform a pre-clustering on sample data to retrieve a suited number if there is none pre-defined by the user.
\item clustering: the actual clustering is carried out by K-Means. The clusters, represented as a vector containing the cluster assignments, is added to our existing matrix $D$ as an additional column. Further information, such as cluster sizes, centers, and densities are used for quality evaluation. We use the sums of squared distances of entries to the center within the cluster (withinss), the sums of squared distances between the cluster centers (betweenss) and the total sums of squares (totalss) to judge the quality of our clusters.
% TODO: Well, how?
\end{itemize}

%  \subsection{Cluster quality evaluation}
%
%%%%%%%%%%% COPY PASTE: TODO: Shorten!!!
%
%Let the following be $m$-dimensional vectors for $m$ metrics, denoted by the index $l$:
%\begin{itemize}
%\item $u_{i}$ the $i$-th user (row in {$D$}) in the data set
%\item $u_{kj}$ the $j$-th user (row in {$D$}) in the $k$-th cluster
%\item $c_{k}$ the $k$-th cluster center
%\item $g$ the global mean
%\end{itemize}
%Also, let the cardinalities be $n$ total users, $n_{clust}$ number of clusters, $n_k$ number of users in the k-th cluster.
%\begin{description}
%\item[withinss]: For each cluster $k$, \emph{withinss} expresses the sum of the squared distances from each user vector to their cluster center:
%\begin{align}
%\textit{withinss}_k = \sum_{j=1}^{n_k}\sum_{l=1}^{m} (c_{kl} - u_{kjl})^2
%\end{align}
%Dividing this value by $n_k$ yields a cluster's variance: $\textit{var}_k = \frac{\textit{withinss}}{n_k}$.
%A lower variance means a denser cluster.
%\item[totalss]: The sum of all squared distances from the individual points to the global mean.
%\begin{align}
%\textit{totalss} = \sum_{i=1}^{n}\sum_{l=1}^{m} (g_{l} - u_{il})^2
%\end{align}
%\item[betweenss]: The sum of the squared distances from the cluster centers to the global minimum, each multiplied with the respective cluster sizes:
%\begin{align}
%\textit{betweenss} = \sum_{k=1}^{n_{clust}} n_k * \sum_{l=1}^{m} (g_l - c_{kl})^2
%\end{align}
%\end{description}
%Dividing \emph{betweenss} by \emph{totalss} yields a measure of variance that can be seen as a cluster quality index $\textit{quality} = \frac{\textit{betweenss}}{\textit{totalss}}$.
%The value of \emph{quality} lies between $0$ (all cluster centers on top of the global mean) and $1$ (all points on top of their cluster centers).
%The closer it is to $1$, the more separated the elements in their clusters are from other cluster centers and the closer they are to their own cluster centers.
%Therefore, this quality index provides a hint whether there are clusters present in the data set and how well K-Means was able to find those.
%It is displayed as a percentage in the Cluster Viewer (see Subsection \ref{subsec:impl:cluster-information-charts}).
%As a limitation, this index typically increases with the number of clusters.
%Thus, in order to judge the results, one needs to consider the number of clusters at the same time.
%
% To get an understanding of potential linear correlations between each of the metrics, we calculate the Pearson correlation index \cite{pearson1895note} using R's \emph{cor} function\footnote{\url{https://stat.ethz.ch/R-manual/R-devel/library/stats/html/cor.html}}.
%%%%%%%%%%%%%%%%%%%



==> sections/problem_statement.tex <==
%!TEX root = ../cluster.tex

\section{Problem Statement}
